De-amortized Cuckoo Hashing: Provable Worst-Case Performance and Experimental Results

Cuckoo hashing is a highly practical dynamic dictionary: it provides amortized constant insertion time, worst case constant deletion time and lookup time, and good memory utilization. However, with a noticeable probability during the insertion of n elements some insertion requires \Omega(log n) time. Whereas such an amortized guarantee may be suitable for some applications, in other applications (such as high-performance routing) this is highly undesirable. Recently, Kirsch and Mitzenmacher (Allerton '07) proposed a de-amortization of cuckoo hashing using various queueing techniques that preserve its attractive properties. Kirsch and Mitzenmacher demonstrated a significant improvement to the worst case performance of cuckoo hashing via experimental results, but they left open the problem of constructing a scheme with provable properties. In this work we follow Kirsch and Mitzenmacher and present a de-amortization of cuckoo hashing that provably guarantees constant worst case operations. Specifically, for any sequence of polynomially many operations, with overwhelming probability over the randomness of the initialization phase, each operation is performed in constant time. Our theoretical analysis and experimental results indicate that the scheme is highly efficient, and provides a practical alternative to the only other known dynamic dictionary with such worst case guarantees, due to Dietzfelbinger and Meyer auf der Heide (ICALP '90).

==> Conclusion.tex <==
\section{Concluding Remarks}\label{sec:Conclusion}

\paragraph{Clocked adversaries.} The worst case guarantees of our dictionary are important if  one wishes to protect against ``clocked adversaries'', as discussed in Section \ref{Sec:intro}. In the traditional RAM model, such guarantees are also sufficient for protecting against such attacks. However, for modern computer architectures the RAM model has
limited applicability, and is nowadays replaced by more accurate hierarchical models (see, for
example, \cite{AggarwalACS87}), that capture the effect of several cache levels. Although our
construction enables the ``brute force'' solution that measures the exact time every operation takes
(see Section \ref{Sec:intro}), a more elegant solution is desirable, which will make a better
utilization of the cache hierarchy. We believe that our dictionary is an important step in this
direction.

\paragraph{Memory utilization.} Our construction achieves memory utilization of essentially
$50\%$. More efficient variants of cuckoo hashing \cite{FotakisPSS05, Panigrahy05, DietzfelbingerW07} circumvent
the $50\%$ barrier and achieve better memory utilization by either using more than two hash
functions, or storing more than one element in each entry. As demonstrated by Kirsch and
Mitzenmacher \cite{KirschM07}, queue-based de-amortization performs very well in practice on these
generalized variants, and it would be interesting to extend our analysis to these variants.

